Equitable and Optimal Transport with Multiple Agents

We introduce an extension of the Optimal Transport problem when multiple costs are involved. Considering each cost as an agent, we aim to share equally between agents the work of transporting one distribution to another. To do so, we minimize the transportation cost of the agent who works the most. Another point of view is when the goal is to partition equitably goods between agents according to their heterogeneous preferences. Here we aim to maximize the utility of the least advantaged agent. This is a fair division problem. Like Optimal Transport, the problem can be cast as a linear optimization problem. When there is only one agent, we recover the Optimal Transport problem. When two agents are considered, we are able to recover Integral Probability Metrics defined by $\alpha$-H\"older functions, which include the widely-known Dudley metric. To the best of our knowledge, this is the first time a link is given between the Dudley metric and Optimal Transport. We provide an entropic regularization of that problem which leads to an alternative algorithm faster than the standard linear program.

==> sections/sec7.tex <==
\section{Experiments}
\label{sec:experiments}

In this section we provide some experiments to illustrate our theoretical analysis and also the performance of our algorithm. In particular, we evaluate our algorithm on Dudley metric with comparison to the algorithm given by~\cite{sriperumbudur2012empirical}. We show our method is a lot faster and still accurate. We provide a new transport interpretation to this metric of interest. 
\paragraph{Accuracy vs Regularization.} 

\begin{figure}[h!]
\centering
\includegraphics[width=0.8\linewidth]{figures/box_plot_accuracy.pdf}
\caption{Accuracy vs Regularization.\label{fig:result_acc}}
\end{figure}


\paragraph{Time vs Dimension.}

\begin{figure}[h!]
\centering
\includegraphics[width=0.3\linewidth]{figures/Time_vs_Dimension.pdf}
\caption{Accuracy vs Regularization.\label{fig:result_acc}}
\end{figure}


The approximation obtained is [PRIMAL formulation]. Explain that this is always bigger than the true value. 



\paragraph{Real Data.}


\section{Conclusion and future work}

In this paper, we defined a new variational problem to deal with multiple costs in Optimal Transport adding the constraints that all the costs must contribute equally to the global transport problem. Primal and dual formulation provides different but coherent interpretations. This helps to understand better the mechanism behind Dudley metric. Following the idea of~\cite{cuturi2013sinkhorn}, we derived an entropic relaxation and an efficient algorithm to approximately compute the solutions to our problem.

We proposed a new way of treating multiple costs in Optimal Transport. There might exist other ways to handle multiple costs and treat them. We leave as further work these other ways. 

==> sections/sec_appli.tex <==
\section{Examples}


\todo{When $c_i(x,y)$ represents the time to transport a unit of good $x$ to a unit of location $y$, then $\max_i\int c_i$ represents the total time to solve the transportation problem: MOT find the fastest way to transport the masses.} 
\todo{Minimise the biggest costs for N days to transport the goods.}
\todo{Matching professors and courses under multiples notations with equal contribution.}
\todo{Asymetric matching: stable mariages problem: in fact it is MOT}
\todo{Appli: learned costs and recomandations for new users using these learned costs}
